VIBEPASS: Can Vibe Coders Really Pass the Vibe Check?

As Large Language Models shift the programming toward human-guided ''vibe coding'', agentic coding tools increasingly rely on models to self-diagnose and repair their own subtle faults -- a capability central to autonomous software engineering yet never systematically evaluated. We present \name{}, the first empirical decomposition that jointly evaluates two coupled tasks: \emph{Fault-Triggering Test Generation (FT-Test)} constructing a discriminative witness that exposes a latent bug, and \emph{Fault-targeted Program Repair (FPR)}, repairing it under varying diagnostic conditions. \name{} pairs competitive programming problems with LLM-generated solutions that pass partial test suites but fail on semantic edge cases, enabling controlled identification of where the diagnostic chain breaks down. Evaluating 12 frontier LLMs, we find that fault-targeted reasoning does not scale with general coding ability. Models produce syntactically valid test inputs at near-ceiling rates yet collapse on discriminative generation, with fault hypothesis generation -- not output validation -- as the dominant bottleneck. Test-guided repair reveals a complementary insight: when self-generated tests successfully witness a fault, the resulting repair matches or outperforms repair guided by externally provided tests, but tests that fail to witness the fault actively degrade repair below unguided baselines. Together, these results reframe the challenge of autonomous debugging: the binding bottleneck is not code synthesis or test validity but fault-target reasoning, a capability that remains deficient across all frontier models. As Large Language Models shift the programming toward human-guided ''vibe coding'', agentic coding tools increasingly rely on models to self-diagnose and repair their own subtle faults -- a capability central to autonomous software engineering yet never systematically evaluated.

==> src/prompts.tex <==
\begin{tcolorbox}[breakable,enhanced, left=-0.5cm, right=-0.5cm, top=2pt, bottom=2pt, enlarge top by=0.1cm, enlarge bottom by=0.1cm]
\begin{quote}
\begin{lstlisting}
You are an excellent software engineer. Your role is to evaluate the correctness of a given python  implementation against its problem specification.

You are provided with:  
- **Problem Description** – Defines the expected behavior of the implementation, including all input variables and constraints.  
- **Python Implementation** – A Python implementation that attempts to solve the problem.

Your task:  
- Analyze the implementation and determine whether it is **functionally correct** for **all valid inputs** defined by the problem description and input constraints.
- If the implementation is **correct**, respond only with program is correct in the 'verdict' tag:
- If the implementation is **incorrect**, response with "program is buggy" in the 'verdict' tag and generate a **failing test case** that exposes the bug in the solution in the 'input' and 'output' tags:

Guidelines for generating the failing test case:
- You only need to produce one failing test case.
- The test input must strictly adhere to all input constraints defined in the problem description.
- Strictly use the same variable identifiers as provided in input constraint
- Match the number, type, name, and order of parameters exactly as in the solution's signature. Do not reorder, add, or remove parameters.
- Ensure the test input can be run directly with the provided solution.
- The input should trigger incorrect behavior such as:
  - Returning the wrong result.
  - Throwing an exception.
  - Producing unexpected output.
- Prefer edge or corner cases likely to reveal logic errors.


Output format:  
- Format your answer as follows:
  - Enclose the verdict in 'verdict' and "verdict' tags.
  - If the implementation is **incorrect**
    - Enclose the test input in 'input' and "input' tags.
    - Enclose the expected output in 'output' and "output' tags.
- For function-call-based testing, provide the test inputs and expected outputs in the below format.
  - Write each function parameter value on its own line using valid Python syntax.
  - Always enclose string inputs/outputs in escaped double quotes (`"`); NEVER output unquoted string literals.
  - Only non-string arguments (e.g., integers, floats, lists) may appear without quotes.
- For code receiving standard input/output stream, respond with the string format of input/output stream

If the implementation is correct:
'verdict'
program is correct
"verdict'

If the implementation is incorrect (function-call-based testing):
'verdict'
program is buggy
"verdict'
'input'
[1,2,3]
"aaabbbccc"
4.0
"input'
'output'
-6
"output'

If the implementation is incorrect (code receiving standard input/output stream):
'verdict'
program is buggy
"verdict'
'input'
3
1 2 3
3 2 1
"input'
'output'
32
"output'

Problem Description:  
{problem}  

Python Implementation:  
{solution}  

Do not generate any reasoning or explanation, only provide the verdict, test input and expected output (if the implementation is incorrect) in the specified format.
\end{lstlisting}
\end{quote}
\label{prompt:p4}
\end{tcolorbox}




\begin{tcolorbox}[breakable,enhanced, left=-0.5cm, right=-0.5cm, top=2pt, bottom=2pt, enlarge top by=0.1cm, enlarge bottom by=0.1cm]
\begin{quote}
\begin{lstlisting}
You are an excellent software engineer. Your role is to expose the bug in the given solution by generating a failing test case based on the problem specification and the provided buggy implementation.  
        
You are provided with:  
- **Problem Description** – Defines the expected behavior of a function, including all input variables and constraints.  
- **Buggy Solution Implementation** – A Python function that is known to be incorrect.  

Your task:  
- Analyze the implementation and produce one failing test case that exposes the bug.  
- The test input must strictly follow all constraints from the problem description.  
- The input should trigger incorrect behavior such as:  
  - Returning the wrong result
  - Throwing an exception
  - Producing unexpected output
- Prefer edge or corner cases likely to reveal logic errors.

Output format:  
- Match the number, type, name, and order of parameters exactly as in the buggy solution's signature.
- Do not reorder, add, or remove parameters.
- Ensure the test input can be run directly with the provided solution.
- Format your answer as follows:
  - Enclose the test input in 'input' and "input' tags.
  - Enclose the expected output in 'output' and "output' tags.
- Do not generate any reasoning or explanation, only provide the test input and expected output in the specified format.

For function-call-based testing, provide the test inputs and expected outputs in 
the below format.
- Write each function parameter value on its own line using valid Python syntax.
- Always enclose string inputs/outputs in escaped double quotes (`"`); NEVER output unquoted string literals.
- Only non-string arguments (e.g., integers, floats, lists) may appear without quotes.

'input'
[1,2,3]
aaabbbccc"
4.0
"input'
'output'
-6
"output'


For code receiving standard input/output stream, respond with the string format of input/output stream in the below format:
'input'
3
1 2 3
3 2 1
"input'
'output'
32
"output'

Problem Description:  
{problem}  

Buggy Solution Implementation:  
{solution}  

Do not generate any reasoning or explanation. Only provide the test input and expected output. Ensure your final response strictly follows the required format.
\end{lstlisting}
\end{quote}
\label{prompt:p4}
\end{tcolorbox}


\begin{tcolorbox}[breakable,enhanced, left=-0.5cm, right=-0.5cm, top=2pt, bottom=2pt, enlarge top by=0.1cm, enlarge bottom by=0.1cm]
\begin{quote}
\begin{lstlisting}
You are an excellent software engineer. Your role is to debug the given solution.

You are provided with:  
- **Problem Description** – Defines the expected behavior of a function, including all input variables and constraints.  
- **Buggy Solution Implementation** – A Python function that is known to be incorrect.

Your task:  
- Analyze the implementation.
- provide the corrected implementation. The corrected implementation should be functionally correct for all valid inputs defined by the problem description and input constraints.

Problem Description:  
{problem}  

Python Implementation (Buggy):  
{solution}  

Output format (Format your answer as follows)
'reasoning'
Briefly describe reasoning for the corrected implementation within 100 words.
"reasoning'
'solution'
```python
WRITE THE CORRECTED IMPLEMENTATION HERE
```
"solution'
\end{lstlisting}
\end{quote}
\label{prompt:p4}
\end{tcolorbox}


\begin{tcolorbox}[breakable,enhanced, left=-0.5cm, right=-0.5cm, top=2pt, bottom=2pt, enlarge top by=0.1cm, enlarge bottom by=0.1cm]
\begin{quote}
\begin{lstlisting}
You are an excellent software engineer. Your role is to debug the given solution based on (but not limited to) the provided failing test case.

You are provided with:  
- **Problem Description** – Defines the expected behavior of a function, including all input variables and constraints.  
- **Buggy Solution Implementation** – A Python function that is known to be incorrect.
- **Failing Test Case** – A failing test case that exposes the bug in the solution.

Your task:  
- Analyze the implementation and failing test case.
- provide the corrected implementation based on the failing test case. The corrected implementation should be functionally correct for all valid inputs defined by the problem description and input constraints.
- If the failing test case is not available (N/A), you shoud generate the corrected implementation based on the best effort to fix the bug.

Problem Description:  
{problem}  

Python Implementation (Buggy):  
{solution}  

Failing Test Case:
[INPUT]
{failing\_test\_input}

[EXPECTED OUTPUT]
{failing\_test\_expected}

Output format (Format your answer as follows)
'reasoning'
Briefly describe reasoning for the corrected implementation within 100 words.
"reasoning'
'solution'
```python
WRITE THE CORRECTED IMPLEMENTATION HERE
```
"solution'
\end{lstlisting}
\end{quote}
\label{prompt:p4}
\end{tcolorbox}


\begin{tcolorbox}[breakable,enhanced, left=-0.5cm, right=-0.5cm, top=2pt, bottom=2pt, enlarge top by=0.1cm, enlarge bottom by=0.1cm]
\begin{quote}
\begin{lstlisting}
You are an excellent software engineer. Your role is to debug the given solution. You should first expose the bug in the given solution by generating a failing test case based on the problem specification and the provided buggy implementation. Then, you should provide the corrected implementation based on the failing test case.

You are provided with:  
- **Problem Description** – Defines the expected behavior of a function, including all input variables and constraints.  
- **Buggy Solution Implementation** – A Python function that is known to be incorrect.  

Your task:  
1. Failing Test Case Generation:
- Analyze the implementation and produce one failing test case that exposes the bug.  
- The test input must strictly follow all constraints from the problem description.  
- The input should trigger incorrect behavior such as:  
  - Returning the wrong result
  - Throwing an exception
  - Producing unexpected output
- Prefer edge or corner cases likely to reveal logic errors.

2. Corrected Implementation Generation:
- Analyze the implementation and the failing test case.
- Identify the bug in the solution using the failing test case (input and expected output) and compare it with the actual output (by mentally running the solution with the failing test case).
- Provide the corrected implementation based on the identified bug. The corrected implementation should be functionally correct for all valid inputs defined by the problem description and input constraints.

Output format (for failing test case generation):  
- Match the number, type, name, and order of parameters exactly as in the buggy solution's signature.
- Do not reorder, add, or remove parameters.
- Ensure the test input can be run directly with the provided solution.
- Format your answer as follows:
  - Enclose the test input in 'input' and "input' tags.
  - Enclose the expected output in 'output' and "output' tags.
- Do not generate any reasoning or explanation, only provide the test input and expected output in the specified format.

For function-call-based testing, provide the test inputs and expected outputs in 
the below format.
- Write each function parameter value on its own line using valid Python syntax.
- Always enclose string inputs/outputs in escaped double quotes (`"`); NEVER output unquoted string literals.
- Only non-string arguments (e.g., integers, floats, lists) may appear without quotes.

'input'
[1,2,3]
"aaabbbccc"
4.0
"input'
'output'
-6
"output'

For code receiving standard input/output stream, respond with the string format of input/output stream in the below format:
'input'
3
1 2 3
3 2 1
"input'
'output'
32
"output'

Output format (for corrected implementation generation):  
'input'
Failing Test Case Input
"input'
'output'
Failing Test Case Expected Output
"output'
'actual\_output'
Failing Test Case Actual Output (by mentally running the solution with the failing test case)
"actual\_output'
'reasoning'
Briefly describe reasoning for the corrected implementation within 100 words.
"reasoning'
'solution'
```python
WRITE THE CORRECTED IMPLEMENTATION HERE
```
"solution'

Problem Description:  
{problem}  

Python Implementation (Buggy):  
{solution}  

Do not generate any reasoning or explanation. Ensure your final response strictly follows the required format.
\end{lstlisting}
\end{quote}
\label{prompt:p4}
\end{tcolorbox}






